Anti-thixotropic dynamics in attractive colloidal dispersions: a shear restructuring driven by elastic stresses

Due to rich rheological properties, dispersions of attractive colloidal particles are ubiquitous in industries. Specifically, upon experiencing a sudden reduction in shear rate, these dispersions may exhibit transient behaviors such as thixotropy-where viscosity increases over time-and anti-thixotropy, characterized by an initial viscosity decrease before reaching a steady state. While thixotropy has been described as a competition between structure buildup and disruption, the mechanisms of anti-thixotropy remain poorly understood. Here, we investigate the anti-thixotropic dynamics of carbon black particles dispersed in oil-a system known for exhibiting anti-thixotropy-through flow step-down experiments. Using a multi-technique approach combining rheology with velocimetry and structural characterizations, we show that viscosity decrease results from a decrease in wall slip concomitant to shear-induced structural rearrangements, indicating a transition from a dynamical network of fractal clusters into a network of loosely connected dense agglomerates. Additionally, after a characteristic anti-thixotropic time $\tau$, a steady flow is reached. This time $\tau$ diverges with increasing shear rate at a critical value corresponding to a Mason number of one, indicating that anti-thixotropy occurs only when colloidal attraction outweighs viscous forces. More precisely, we show that the structural rearrangement underpinning the viscosity decrease is mediated by elastic stresses $\sigma_e$, such that $\tau \propto \sigma_e^{-3}$. Finally, on long time scales, the steady state is linked to a microstructure with nearly zero yield stress, indicating a loss of flow memory. These findings provide a mechanism for anti-thixotropy and suggest pathways for controlling viscosity and yield stress in attractive colloidal dispersions.

==> AncienneIntro.tex <==
% Definition and examples of yield stress fluids
Yield stress fluids encompass a wide range of soft materials, including emulsions (\emph{e.g.}, mayonnaise), suspensions (\emph{e.g.}, fresh cement paste and drilling muds), and foams (\emph{e.g.}, shaving cream). These materials exhibit a dual behavior depending on the applied stress $\sigma$ relative to a critical value termed as "yield stress" $\sigma_y$~\cite{Coussot2014,Bonn2017,Nelson2017}. When $\sigma < \sigma_y$, they behave like solids, but they flow like liquid fluids when $\sigma > \sigma_y$. The transition between solid and fluid states is fully shear-reversible, provided there are no chemical transformations or composition changes (\emph{e.g.}, drying) during the experimental timescale.

% Simple and thixotropic yield stress fluids
The yield stress can typically be measured via creep tests with varying stress magnitudes in order to determine whether the material flows under a given stress. For "simple" ({i.e.,}, non-thixotropic) yield stress fluids, the viscosity continuously diverges as $\sigma$ approaches $\sigma_y$, allowing steady flow conditions to be achieved~\cite{Møller2009}. These fluids, typically high-volume fraction suspensions of weakly interacting non-Brownian particles, progressively jam near $\sigma_y$. In contrast, "complex" or thixotropic yield stress fluids, such as attractive colloidal suspensions, exhibit an abrupt transition, with the viscosity that jumps from a finite value under steady flow to infinity in the solid regime~\cite{Coussot2002,Coussot2002a}. In these fluids, solid-like properties are rather attributed to a percolated network of attractive particles with a fractal-like organization.

% Heterogeneous flow
Measuring the rheological properties of yield stress fluids near $\sigma_y$ is challenging as heterogeneous flow profiles, i.e., variations of the local shear rate in the sample, may occur~\cite{Ewoldt}, including wall slip or shear banding~\cite{Divoux2015, gibaud2008, gibaud2016}. In particular, when the material is put to flow from rest, the yielding transition involves long transient responses, evolving from a highly heterogeneous flow to linear velocity profiles~\cite{Divoux2016}. The time scale of this phenomenon was defined as the "fluidization time" and generally decreases as a power law of the applied stress for simple yield stress fluids~\cite{Divoux2010,Divoux2012} but shows an exponential dependence for thixotropic yield stress fluids~\cite{Gibaud2010}.
%In coaxial cylinder geometry, the local stress $\sigma(r) \propto 1 / r^2$, $r$ being the radial position, may causes parts of the fluid to be below $\sigma_y$. Shear banding is correlated with the magnitude of particle interactions~\cite{Chaudhuri2012, Liberto2020}.

% Thixotropy
Compared to simple yield stress fluids, thixotropic yield stress fluids exhibit additional complexity due to their microstructure and viscosity depending on both time and shear magnitude~\cite{Barnes1997, Mewis2009, Joshi2018}. Strictly speaking, thixotropy refers to a time-dependent increase in viscosity after a decrease in shear stress or shear rate. This behavior stems from the equilibrium size of the particle aggregates, influenced by competing attraction and shear forces. Recent studies, including numerical simulations~\cite{Varga2018} and experiments~\cite{Bauland2024}, have shown that the aggregate size has an upper limit where they form dynamical networks below a critical shear rate. In this case, transient dynamics following a shear step results from a competition between the spontaneous aging of the microstructure and its shear-induced rejuvenation~\cite{Gibaud2010, Sprakel2011}.

%The transient response of thixotropic fluids is well captured by structural kinetics model. In this framework, the competition between the structure build-up and destruction under shear is accounted by introducing kinetics equations for a structural parameter $\lambda$, which varies between 0 and 1 for a totally broken or fully developed structure, respectively~\cite{Dullaert2006}.
%Thixotropic yield stress fluids are sometimes referred as "complex" yield stress fluids. Indeed, the viscosity bifurcation when $\sigma \longrightarrow \sigma_y$ implies that no steady state can be reached when the applied shear $\sigma \leq \sigma_y$.
% Efficiency of these models to reproduce lies in the arbitrary choice of kinetics equations for $\lanbda$, hindering further understanding.

% Anti-tixotropy and shear-structuration
In contrast to thixotropy, colloidal suspensions can also exhibit "antithixotropy" or "rheopexy", defined as a decrease of viscosity following a shear step-down. Antithixotropy has been reported for several attractive systems at moderate shear rates and has been attributed to the formation of dense, large agglomerates that reduce the effective volume fraction of the suspension~\cite{Essadik2021, Osuji2008, Narayanan2017, Ovarlez2013a, Hipp2019, Wang2022}. antithixotropic behavior has also been referred to as "rheomalaxis" by reference to this long transient state leading to the formation of dense agglomerates~\cite{Barnes1997}. Disruption of these agglomerates at higher shear rates can lead to apparent shear-thickening, provided the aggregates formed at higher shear are fractal~\cite{Osuji2008}. Such dramatic structuring of colloidal suspensions offers the possibility to tune at will the viscosity and the yield stress of colloidal suspensions~\cite{Ovarlez2013a,Jiang2022}. 

% Pb of or study --> no mechanisms in contrast with confining conditions
Under confinement—when the gap size is small relative to the particle size—shear-induced structuring can lead to the formation of log-rolling structures~\cite{Grenard2011,Varga2019}. The formation of these large, anisotropic structures were attributed to hydrodynamic coupling between the flocs and the confining boundaries that triggers viscous eddies. As previously discussed, shear-induced densification, termed antithixotropy, can also occur in non-confining conditions. Yet, despite numerous studies on this phenomenon, the specific microstructural scenario underlying the stress decrease, as well as the physical mechanisms involved, remain to be clarified. 

% Scope and aim of the study
In this study, we investigate the antithixotropic response of carbon black (CB) particles in oil—a system known to exhibit antithixotropy\cite{Richards2023}—by performing step-down of shear rate experiments. During rheometric tests, we use ultrasonic speckle velocimetry (USV) to distinguish between local and bulk contribution to the measured stress and tackle the real dynamics of the antithixotropic response at fixed shear rate. We use a combination of rheo-ultra small angle X-ray scattering (USAXS) and rheo-electrical impedance spectroscopy (EIS) measurements to probe the hierarchical structure of CB suspensions. First, USV reveals that the decrease in stress upon a step-down of shear rate is preceded by a slipping regime, during which the material organizes into a dynamic fractal network. As shear propagates through the geometry gap, this fractal structure continuously rearranges into dense and large agglomerates, as confirmed by ultra-small angle X-ray scattering (USAXS) and electrical impedance spectroscopy (EIS). The characteristic time of the antithixotropic response is found to increase exponentially with the applied shear rate, up to a critical threshold. This critical shear rate is interpreted as critical Mason number, where clusters become effectively sticky relative to shear forces. Using flow cessation or "stress jump" experiments, we show that the restructuring of the fractal structure relies on elastic stresses that deform the  partially connected fractal network. Interestingly, the steady state associated with the antithixotropic response results in a single structuring of the suspensions with a vanishing small yield stress, indicating a 'partial memory' of the flow in this regime. 
